Four new deeply-eclipsing white dwarfs in ZTF

We present the results of a search for deeply-eclipsing white dwarfs in the ZTF Data Release 4. We identify nine deeply-eclipsing white dwarf candidates, four of which we followed up with high-cadence photometry and spectroscopy. Three of these systems show total eclipses in the ZTF data and our follow-up APO 3.5-meter telescope observations. Even though the eclipse duration is consistent with sub-stellar companions, our analysis shows that all four systems contain a white dwarf with low-mass stellar companions of ~0.1 Msol. We provide mass and radius constraints for both stars in each system based on our photometric and spectroscopic fitting. Finally, we present a list of 41 additional eclipsing WD+M candidates identified in a preliminary search of ZTF DR7, including 12 previously studied systems. We identify two new candidate short-period, eclipsing, white dwarf-brown dwarf binaries within our sample of 41 WD+M candidates based on PanSTARRS colors.

==> equations/binary_mass_function.tex <==
\begin{equation}
\frac{(M_{2}\ \text{sin}\ i)^3}{(M_1+M_{2})^2} = \frac{PK^3}{2 \pi G},
\label{eqn:binary_mass_function}
\end{equation}

